Sequentiality of String-to-Context Transducers

Transducers extend finite state automata with outputs, and describe transformations from strings to strings. Sequential transducers, which have a deterministic behaviour regarding their input, are of particular interest. However, unlike finite-state automata, not every transducer can be made sequential. The seminal work of Choffrut allows to characterise, amongst the functional one-way transducers, the ones that admit an equivalent sequential transducer. In this work, we extend the results of Choffrut to the class of transducers that produce their output string by adding simultaneously, at each transition, a string on the left and a string on the right of the string produced so far. We call them the string-to-context transducers. We obtain a multiple characterisation of the functional string-to-context transducers admitting an equivalent sequential one, based on a Lipschitz property of the function realised by the transducer, and on a pattern (a new twinning property). Last, we prove that given a string-to-context transducer, determining whether there exists an equivalent sequential one is in coNP.

==> 066-correctness.tex <==
% !TEX root = ./main.tex

\begin{lemma}[Correctness of $\D$]\label{r:corr}
  For all $\qB \in \dom(\bar{F})$ such that $\iB \ttrans[\D]{u}{c} \qB$,
    $\tinit \act u [\eps] = \Delta_{\qB} c [\eps]$
    and for all $q \in \dom(\Delta_{\qB}) \cap \dom(\tfinal)$,
      $\tfinal(q) \cdot \Delta_{\qB}(q) = \bar{F}(\qB)$.
\end{lemma}

\begin{proof}[Proof Sketch]
  \red{TODO}
\end{proof}


==> 067-boundedness.tex <==
% !TEX root = ./main.tex

\newcommand{\QQ}{\ensuremath{|Q|^{|Q|}}}

By convention, we consider that $|\bot| = 0$.

%--------------------------------------------------------------------------------------------------

\begin{lemma}[Boundedness of $\D$]\label{r:boundedness}
  \note{\red{State this in a simpler way to avoid having to define $\base$ ?}}
  For all $\qB = (x', \Delta', H') \in \Qb$
    such that $\iB \ttrans[D]{u}{c} \qB$,
    the following assertions are satisfied:
  \begin{itemize}
    \item $|x'| \leq \base \QQ$,
    \item for all $(q,d) \in \Delta'$, $|d| \leq \base \QQ$,
    \item $|word(H')| < \QQ$.
  \end{itemize}
\end{lemma}

\begin{proof}[Proof Sketch]
  \red{TODO}
\end{proof}


==> 130-annex-lipschitz-twinning.tex <==
% !TEX root = ./main.tex

